BIP! NDR (NoDoiRefs): A Dataset of Citations From Papers Without DOIs in Computer Science Conferences and Workshops

In the field of Computer Science, conference and workshop papers serve as important contributions, carrying substantial weight in research assessment processes, compared to other disciplines. However, a considerable number of these papers are not assigned a Digital Object Identifier (DOI), hence their citations are not reported in widely used citation datasets like OpenCitations and Crossref, raising limitations to citation analysis. While the Microsoft Academic Graph (MAG) previously addressed this issue by providing substantial coverage, its discontinuation has created a void in available data. BIP! NDR aims to alleviate this issue and enhance the research assessment processes within the field of Computer Science. To accomplish this, it leverages a workflow that identifies and retrieves Open Science papers lacking DOIs from the DBLP Corpus, and by performing text analysis, it extracts citation information directly from their full text. The current version of the dataset contains more than 510K citations made by approximately 60K open access Computer Science conference or workshop papers that, according to DBLP, do not have a DOI.

==> abstract.tex <==
\abstract{The amount of textual data produced nowadays is constantly increasing, as the number and variety of both new and reproduced textual information %created by humans and (lately) also by bots 
is unprecedented. Storing, handling and querying such high volumes of textual data have become more challenging than ever and both research and industry have been using various alternatives, ranging from typical Relational Database Management Systems to specialised text engines and NoSQL databases, in an effort to cope with the volume. However, all these decisions are, largely, based on experience or personal preference for one system over another, since there is no performance comparison study that compares the available solutions regarding full-text search and retrieval. In this work, we fill this gap %in the literature 
by systematically comparing four popular databases in full-text search scenarios and reporting their performance across different datasets, full-text search operators and parameters. To the best of our knowledge, our study is the first %to go beyond the comparison of characteristics, like expressiveness of the query language or popularity, and 
to actually compare popular relational, NoSQL and textual data stores, in terms of retrieval efficiency for full-text search. Moreover, our findings quantify the differences in full-text search performance between the examined solutions and reveal both anticipated and  less anticipated results.}
